Expressions of Sentiments During Code Reviews: Male vs. Female

Background: As most of the software development organizations are male-dominated, female developers encountering various negative workplace experiences reported feeling like they "do not belong". Exposures to discriminatory expletives or negative critiques from their male colleagues may further exacerbate those feelings. Aims: The primary goal of this study is to identify the differences in expressions of sentiments between male and female developers during various software engineering tasks. Method: On this goal, we mined the code review repositories of six popular open source projects. We used a semi-automated approach leveraging the name as well as multiple social networks to identify the gender of a developer. Using SentiSE, a customized and state-of-the-art sentiment analysis tool for the software engineering domain, we classify each communication as negative, positive, or neutral. We also compute the frequencies of sentiment words, emoticons, and expletives used by each developer. Results: Our results suggest that the likelihood of using sentiment words, emoticons, and expletives during code reviews varies based on the gender of a developer, as females are significantly less likely to express sentiments than males. Although female developers were more neutral to their male colleagues than to another female, male developers from three out of the six projects were not only writing more frequent negative comments but also withholding positive encouragements from their female counterparts. Conclusion: Our results provide empirical evidence of another factor behind the negative work place experiences encountered by the female developers that may be contributing to the diminishing number of females in the SE industry.

==> Images/number-contributors.tex <==
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|l|R{1.1cm}|r|r|R{1cm}|}
\hhline{------}
\graycell{Project} & Managed by & \# contributors & \% female & \# core & \% core (female) \\
\hline
Android & Google & 968 & 6.19\% & 258 & 3.87\% \\ 
\hline 
Chromium OS & Google & 1,007 & 8.74\% & 151 & 3.97\% \\ 
%\hline 
%Coreboot & Community & 111 & 4.50\% & 21 & 0.00\%  \\ 
\hline 
Couchbase & Couchbase & 165 & 9.69\% & 24 & 4.17\%  \\ 

\hline 
Go & Google & 220 & 19.09\% & 90 & 7.77\% \\ 
\hline 

%ITK / VTK & Kitware & 174 & 3.44\% & 33 & 3.03\% \\ 
%\hline 
LibreOffice & Community & 344 & 8.14\% & 68 & 1.47\% \\ 
\hline 

OmapZoom & TI & 425 & 7.06\% & 60 & 11.66\% \\ 

\hline 
OVirt & Redhat & 220 & 9.54\% & 34 & 2.94\% \\ 
\hline 

Qt & Digia & 736 & 3.12\% & 159 & 3.14\% \\ 
\hline 

Typo3 & Community & 318 & 3.77\% & 73 & 4.10\% \\ 
\hline 

Whamcloud & Intel & 140 & 7.85\% & 19 & 0.00\% \\ 
\hline 
%Wireshark & Community & 181 & 1.66\% & 55 & 1.81\% \\ 
%\hline 

\end{tabular} 

}

==> Tables/number-contributors.tex <==
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|l|R{1.1cm}|r|r|R{1cm}|}
\hhline{------}
\graycell{Project} & Managed by & \# contributors & \% female & \# core & \% core (female) \\
\hline
Android & Google & 968 & 6.19\% & 258 & 3.87\% \\ 
\hline 
Chromium OS & Google & 1,007 & 8.74\% & 151 & 3.97\% \\ 
%\hline 
%Coreboot & Community & 111 & 4.50\% & 21 & 0.00\%  \\ 
\hline 
Couchbase & Couchbase & 165 & 9.69\% & 24 & 4.17\%  \\ 

\hline 
Go & Google & 220 & 19.09\% & 90 & 7.77\% \\ 
\hline 

%ITK / VTK & Kitware & 174 & 3.44\% & 33 & 3.03\% \\ 
%\hline 
LibreOffice & Community & 344 & 8.14\% & 68 & 1.47\% \\ 
\hline 

OmapZoom & TI & 425 & 7.06\% & 60 & 11.66\% \\ 

\hline 
OVirt & Redhat & 220 & 9.54\% & 34 & 2.94\% \\ 
\hline 

Qt & Digia & 736 & 3.12\% & 159 & 3.14\% \\ 
\hline 

Typo3 & Community & 318 & 3.77\% & 73 & 4.10\% \\ 
\hline 

Whamcloud & Intel & 140 & 7.85\% & 19 & 0.00\% \\ 
\hline 
%Wireshark & Community & 181 & 1.66\% & 55 & 1.81\% \\ 
%\hline 

\end{tabular} 

}

==> Tables/table-contributions.tex <==
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|l|r|r|r|r|r|}
\hhline{-------}
\multirow{2}{*}{ \graycell{Project}} & \multicolumn{3}{|c|}{ \graycell{Review requests/month}} & \multicolumn{3}{|c|}{\graycell{Code churn / month}} \\
\hhline{~------}
& \graycell{Male} & \graycell{Female} & \graycell{$p (MWU)$} & \graycell{Male} & \graycell{Female} &\graycell{ $p (MWU)$} \\
\hline
Android & 2.5 & 1.9 & 0.15 & 268 & 154 &  0.13 \\ 
\hline 
Chromium OS & 4.0 & 3.6 & 0.77 & 481 & 696 &  0.16 \\ 
%\hline 
%Coreboot & 3.0 & 3.6 & 0.52 & 419 & 429 &  0.99 \\ 
\hline 
Couchbase & 8.9 & 7.1 & 0.19 & 1168 & 947 &  0.63 \\ 

\hline 
Go & 1.8 & 7.2 & \textbf{0.004} & 170 & 559 &  \textbf{0.04} \\ 
\hline 

%ITK / VTK & 2.6 & 1.2 & 0.27 & 904 & 1079 &  0.63 \\ 
%\hline 
LibreOffice & 3.0 & 1.8 & 0.08 & 352 & 86 &  \textbf{0.003} \\ 
\hline 

OmapZoom & 3.6 & 4.2 & 0.99 & 321 & 352 &  0.66 \\ 

\hline 
OVirt & 6.4 & 6.7 & 0.84 & 570 & 301 &  0.13 \\ 
\hline 

Qt & 2.78 & 3.22 & 0.74  & 263 & 277 & 0.66\\ 
\hline 


Typo3 & 1.6 & 3.7 & 0.25 & 227 & 890 &  0.27 \\ 
\hline 

Whamcloud & 1.5 & 2.0 & 0.94 & 263 & 277 &  0.60 \\ 
\hline 
%Wireshark & 2.0 & 0.92 & 0.44 & 316 & 225 &  0.71 \\ 
%\hline 

\end{tabular} 

}

==> Tables/table-discrimination.tex <==
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|l|r|r|r|r|r|}
\hhline{-------}
\multirow{2}{*}{ \graycell{Project}} & \multicolumn{3}{|c|}{ \graycell{Acceptance rate}} & \multicolumn{3}{|c|}{\graycell{Review Interval (hrs)}} \\
\hhline{~------}
& \graycell{Male} & \graycell{Female} & \graycell{$p ({\chi}^2)$} & \graycell{Male} & \graycell{Female} &\graycell{ $p (MWU)$} \\
\hline
Android & 88.1 & 77.6 & $<$\textbf{0.001} & 20.1 & 69.5 &  $<$\textbf{0.001} \\ 
\hline 
Chromium OS & 91.4\% & 90.1\% &\textbf{ 0.001} & 31.1 & 31.3 &  0.19 \\ 
%\hline 
%Coreboot & 3.0 & 3.6 & 0.52 & 419 & 429 &  0.99 \\ 
\hline 
Couchbase & 92.1\% & 90.4\% & \textbf{0.015} & 17.5 & 21.6 &  $<$\textbf{0.001} \\ 

\hline 
Go & 91.6\% & 90.8\% & 0.44 & 16.6 & 16.7 &  0.46\\ 
\hline 

%ITK / VTK & 2.6 & 1.2 & 0.27 & 904 & 1079 &  0.63 \\ 
%\hline 
LibreOffice & 92.3\% & 83.5\% & $<$\textbf{0.001} & 23.3 & 72.4 &  $<$\textbf{0.001} \\ 
\hline 

OmapZoom & 75.05\% & 75.8\% & 0.45 & 160.1 & 146.9 &  0.70 \\ 

\hline 
OVirt & 88.1\% & 91.1\% &$<$\textbf{0.001} &49.4 & 47.9 &  0.15 \\ 
\hline 

Qt & 90.5\%& 93.8\% & $<$\textbf{0.001} & 32.7 & 19.8 & $<$\textbf{0.001}\\ 
\hline 


Typo3 & 91.1\% & 92.0\% & 0.36 & 25.9 & 12.1 &  $<$\textbf{0.001} \\ 
\hline 

Whamcloud & 78.8\% & 78.4\% & 0.89 & 367.9 & 356.9 &  0.54 \\ 
\hline 
%Wireshark & 2.0 & 0.92 & 0.44 & 316 & 225 &  0.71 \\ 
%\hline 

\end{tabular} 

}
